Self-Correcting Neural Networks For Safe Classification

Classifiers learnt from data are increasingly being used as components in systems where safety is a critical concern. In this work, we present a formal notion of safety for classifiers via constraints called safe-ordering constraints. These constraints relate requirements on the order of the classes output by a classifier to conditions on its input, and are expressive enough to encode various interesting examples of classifier safety specifications from the literature. For classifiers implemented using neural networks, we also present a run-time mechanism for the enforcement of safe-ordering constraints. Our approach is based on a self-correcting layer, which provably yields safe outputs regardless of the characteristics of the classifier input. We compose this layer with an existing neural network classifier to construct a self-correcting network (SC-Net), and show that in addition to providing safe outputs, the SC-Net is guaranteed to preserve the classification accuracy of the original network whenever possible. Our approach is independent of the size and architecture of the neural network used for classification, depending only on the specified property and the dimension of the network's output; thus it is scalable to large state-of-the-art networks. We show that our approach can be optimized for a GPU, introducing run-time overhead of less than 1ms on current hardware -- even on large, widely-used networks containing hundreds of thousands of neurons and millions of parameters.

==> figures/sr-net_flow.tex <==
% !TEX root=../main.tex
\centering
\noindent

\scalebox{0.85}{%
\begin{tikzpicture}[
vector/.style={
    rectangle, 
    draw=black!60, 
    fill=white, 
    thin, 
    minimum size=7mm},
function/.style={
    rectangle, 
    draw=black!80, 
    fill=white, 
    thin, 
    minimum size=0.5in, 
    inner sep=0.25in},
groupnode/.style={
    rectangle, 
    draw=black, 
    fill=black!5, 
    thin, 
    minimum size=2cm,
    inner sep=0.125in},
]

%Nodes
\node[vector]    (x)                        {$x$};
\node[function]  (f)      [right=of x]      {original network $f$};
\node[vector]    (y)      [right=of f]      {$y$};
\node[function]  (repair) [right=of y]      {\Frepair{$\properties ~~,~~ x ~~,~~ y$}};
\node[vector]    (yp)     [right=of repair] {$y'$};

\begin{scope}[on background layer]
    \node[groupnode, fit=(f) (repair), label={transformed neural network $\arnet$}](fphi) {};
\end{scope}

%Lines
\draw[thick, ->] (x.east) -- (f.west);
\draw[thick, ->] (f.east) -- (y.west);
\draw[thick, ->] (y.east) -- (repair.west);
\draw[thick, ->] (repair.east) -- (yp.west);
\draw[thick, ->] (x.east) 
    -- ($(x.east)+(0.5,0)$) 
    -- ($(x.east)+(0.5,0.95)$)
    -- ($(y.east)+(0.5,0.95)$)
    -- ($(y.east)+(0.5,0.25)$)
    -- ($(repair.west)+(0,0.25)$);
\end{tikzpicture}}


==> outline.tex <==
% !TEX root=./main.tex

\section*{Outline}

\paragraph{Introduction.}
Introduce the problem of safety in neural networks.
Talk about both robustness and general safety properties, e.g., the ones in ACAS.
Introduce some of the prior work on safety certification; taxonomize, and place ourselves.
In particular point out the cost of static analysis, and how encoding properties in the loss function can be brittle.
Point out that we propose on-line repair.
While the concept is simple, we explore the challenges of actually implementing this and show how it can be done.
We demonstrate our approach on a handful of applications that have been studied before in the literature.

\paragraph{Related Work.}
Go into a bit more depth on the related work that's relevant to this paper.

\paragraph{Problem Setting.}
Lay out a formalization of the types of properties we will handle.
Explain the motivation for restricting generality to ordering constraints over general polytopes.
Show how previous problems can be formulated in this way.

\paragraph{Self-Repair.}
This is where we describe our approach.
Start at a high level describing the main idea: (1) check which preconditions are satisfied to collect the relevant postconditions; (2) modify the output of the network to be consistent with the required post-conditions.
The main challenge is (2); with the primary challenges being (a) how do we handle disjunctions, and (b) how do we repair a property given there are no disjunctions (assuming the property is satisfiable).
We will start with (b) and then show how to handle (a).
We will defer to the next section to describe how this can be efficiently encoded to run on a GPU in a neural network.

\paragraph{Implementation.}
This is where we get into more of the details of how this is possible within a standard machine learning framework.
We discuss the representations used and the specific algorithms we use to solve the sub-problems identified in the previous section.

\paragraph{Evaluation.}
Provide experiments on ACAS, some of the other related problems, and synthetic data that gets at scalability.
Compare to ART, and other relevant approaches.
Look at overhead, scalability, and success at certification.

\paragraph{Discussion.}
Here we can discuss some of the other ideas that can be used to modify our approach to help with various trade-offs, e.g., the question of where to do the work of SMT solving.
We can also talk about the concept of training vs. post-hoc application of repair, and what happens if the guard rails are taken off.

\paragraph{Conclusion.}
The standard conclusion that just recaps the important contributions and gives some thoughts on future directions.


==> proofnotmaximal.tex <==
% !TEX root=./main.tex

\section{Proof of notmaximal procedure}
\label{sec:proofnotmax}

\begin{lstlisting}[mathescape=true][language=Python]
$\color{red}\{y \in Arr_d(\mathbb{R}) \wedge I \in 2^{\mathbb{N}} \wedge 
\forall i \in I. 0 \leq i < d \wedge |I| < d\}$
repair(y,I):
	m := [1 at each index in I, 0 elsewhere]
$\color{red}\{m \in Arr_d(\{0,1\}) \wedge \forall i \in [0,d). (m[i] = 1 \leftrightarrow i \in I 
\wedge m[i] = 0 \leftrightarrow i \notin I)  \}$
	ySorted := sort(y)
$\color{red}\{\perm(ySorted,y) \wedge \forall i,j \in [0,d). i \leq j \rightarrow ySorted[i] \geq ySorted[j] \}$
	yPerm := argsort(y)
$\color{red}\{ yPerm \in Arr_d(\mathbb{N}) \wedge \forall i \in [0,d) ySorted[i] = y[yPerm[i]]\}$
	yPermInv := invert_perm(yPerm)
$\color{red}\{\perm(yPermInv,yPerm) \wedge \forall i \in [0,d). (yPermInv[yPerm[i]] = i 
\wedge yPermInv[i] = \idx(yPerm,i))\}$
	m' := m[yPerm]
$\color{red}\{\perm(m',m) \wedge \forall i \in [0,d). m'[i] = m[yPerm[i]] \}$
	r := argmin(m')
$\color{red}\{m'[r] = 0 \wedge \forall i \in [0,r). m'[i] = 1 \}$
	yFront := ySorted[:r+1]
$\color{red}\{yFront \in Arr_{r+1}(\mathbb{R}) \wedge \forall i \in [0,r+1). yFront[i] = ySorted[i]\}$
	yBack := ySorted[r+1:]
$\color{red}\{yBack \in Arr_{d-r-1}(\mathbb{R}) \wedge \forall i \in [r+1,d). yBack[i] = ySorted[i]\}$
	yRoll := roll(yFront, -1)
$\color{red}\{\perm(yRoll,yFront) \wedge \forall i \in [1,r+1). yRoll[i] = yFront[i+1] \wedge yRoll[r] = yFront[0] \}$
$\color{red}\{\forall i \in [0,r+1). yRoll[r] \geq yRoll[i] \}$
	yConcat := concat(yRoll, yBack)
$\color{red}\{\perm(yConcat,ySorted) \wedge \forall i \in [0,d). yConcat[r] \geq yConcat[i] \}$
	yFinal := yConcat[yPermInv]
$\color{red}\{\perm(yFinal,yConcat) \wedge \forall i \in [0,d). yFinal[i] = yConcat[yPermInv[i]]\}$
$\color{red}\{\perm(yFinal,y) \wedge r=yPermInv[i_0] \wedge m'[r] = 0 \wedge \forall i \in [0,d). yFinal[i_0] \geq yFinal[i]\}$
$\color{red}\{\perm(yFinal,y) \wedge m[yPerm[r]] = 0 \wedge \forall i \in [0,d). yFinal[i_0] \geq yFinal[i]  \}$
$\color{red}\{\perm(yFinal,y) \wedge m[yPerm[yPermInv[i_0]]] = 0 \wedge \forall i \in [0,d). yFinal[i_0] \geq yFinal[i]  \}$
$\color{red}\{\perm(yFinal,y) \wedge m[yPerm[\idx(yPerm,i_0)]] = 0 \wedge \forall i \in [0,d). yFinal[i_0] \geq yFinal[i]  \}$
$\color{red}\{\perm(yFinal,y) \wedge m[i_0] = 0 \wedge \forall i \in [0,d). yFinal[i_0] \geq yFinal[i]  \}$
$\color{red}\{\perm(yFinal,y) \wedge i_0 \notin I \wedge \forall i \in I. yFinal[i] \leq yFinal[i_0]\}$
$\color{red}\{\perm(yFinal,y) \wedge \forall i \in I. yFinal[i] \; is \; not \; maximal\}$
	return yFinal
$\color{red}\{\perm(yFinal,y) \wedge \forall i \in I. yFinal[i] \; is \; not \; maximal\}$


\end{lstlisting}



==> section_correctness.tex <==
% !TEX root=./main.tex

\section{Safety and Accuracy}
\label{sec:correctness}

In this section, we present the two main theorems of our work.
First, we show that the approach presented in Section~\ref{sec:repair}
yields a self-repairing transformer; i.e., \Fselfrepair satisfies the properties from
Defintion~\ref{def:sr-transformer}. 
Second, we prove that the network transformer we propose also satisfies transparency
(Property~\ref{thm:transparency}), ensuring a repaired network is at least as accurate as
the original network (Theorem~\ref{thm:preservation}).

\subsection{\ls`SR` is a Self-Repairing Transformer}
\label{sec:proof_safety}

We start by proving that the transformer presented in Algorithm~\ref{alg:self_repair}, \Fselfrepair,
is self-repairing; i.e., it satisfies Properties~\ref{def:sr-transformer}\ref{thm:safety}
and~\ref{def:sr-transformer}\ref{thm:forewarning}.
Recall that this means that $\arnet$ will either return safe outputs vectors, or in the event that $\Phi$ is inconsistent at a point, and \emph{only} in that event, return $\bot$.

Let $x : \mathbb{R}^n$ be an arbitrary vector.
If $\Phi(x, f(x))$ is initially satisfied, the \arlayer does not modify
the original output $y = f(x)$, and Properties~\ref{def:sr-transformer}\ref{thm:safety}
and \ref{def:sr-transformer}\ref{thm:forewarning} are trivially satisfied.
If $\Phi(x, f(x))$ does not hold, we will rely on two key properties of \Fsolve and \Freorder to establish that \Fselfrepair is self-repairing.
The first, Property~\ref{thm:solvespec}, requires that \Fsolve either return $\bot$, or else return ordering constraints that are sufficient to establish $\Phi$.

\begin{Property}[\Fsolve]
\label{thm:solvespec}
Let $\Phi$ be a set of safety properties, $x : \mathbb{R}^n$ and $y : \mathbb{R}^m$ two
vectors.\\
Then $q = \Fsolve(\Phi, x, y)$ satisfies the following properties:

\begin{enumerate}[label=(\roman*),font=\itshape]
\item \label{thm:solvebot} $q = \bot \Longleftrightarrow \forall y'~.~\lnot \Phi(x, y')$
\item \label{thm:solverep} $q \neq \bot \implies (~\forall y'~.~q(y') \implies \Phi(x, y')~)$
\end{enumerate}
\end{Property}
\begin{proof}
The first observation is that the list of ordering constraints in
$Q_p := \Fprioritize(Q_x, y)$ accurately models
the initial set of properties $\Phi$, i.e.,
\begin{equation}
\label{eqn:prspec}
\forall y'~.~\Phi(x, y') \Longleftrightarrow (~\exists q \in Q_p~.~q(y')~)
\end{equation}
This stems from the definition of the disjunctive normal form,
and from the fact that \Fprioritize only performs a permutation of the disjuncts.

We also rely on the following loop invariant, stating that all disjuncts considered so far, when iterating over \linebreak
$\Fprioritize(Q_x, y)$, were unsatisfiable:
\begin{equation}
\label{eqn:solve_loopinv}
\forall q \in Q_p~.~\idx(q, Q_p) < \idx(q_i, Q_p)
\implies (~\forall y~.~\neg q(y)~)
\end{equation}

Here, $\idx(q,Q_p)$ returns the index of constraint $q$ in the list $Q_p$.
This invariant is trivially true when entering the loop,
since the current $q_i$ is the first element of the list.
Its preservation relies on $\Fissat(q)$ correctly determining whether $q$ is satisfiable, i.e., $\Fissat(q) \Longleftrightarrow \exists y~.~q(y)$~\cite{graphissat}.

Combining these two facts, we can now establish that \Fsolve satisfies \ref{thm:solvespec}\ref{thm:solvebot} and \ref{thm:solvespec}\ref{thm:solverep}.
By definition, $\Fsolve(\Phi, x, y)$ outputs $\bot$ if and only if it traverses
the entire list $Q_p$, never returning a $q_i$.
From loop invariant~\ref{eqn:solve_loopinv}, this is equivalent to
$\forall q \in Q_p.~\forall y'.~\lnot q(y')$, which finally yields
property~\ref{thm:solvespec}\ref{thm:solvebot} from
equation~\ref{eqn:prspec}.
Conversely, if $\Fsolve(\Phi, x, y)$ outputs $q \neq \bot$, then $q \in Q_p$.
We directly obtain property~\ref{thm:solvespec}\ref{thm:solverep} as,
for any $y' : \mathbb{R}^m$, $q(y')$ implies that $\Phi(x, y')$ by application
of equation~\ref{eqn:prspec}
\end{proof}

Next, Property~\ref{thm:reorderspec} states that $\Freorder$ correctly permutes the output of the network to satisfy the constraint that it is given.
Combined with Property~\ref{thm:solvespec}, this is sufficient to show that \Fselfrepair is a self-repairing transformer (Theorem~\ref{thm:sr-sound}).

\begin{Property}[\Freorder]
\label{thm:reorderspec}
Let $q$ be a satisfiable ordering constraint, and $y : \mathbb{R}^m$ a vector.
Then $\Freorder(q, y)$ satisfies $q$.
\end{Property}
\begin{proof}
Let $y_i < y_j$ be an atom in $q$. Reusing notation from Algorithm~\ref{alg:repair:reorder}, let $y' = \Freorder(q, y)$, $y^s := \Fdescsort(y)$, and $\pi := \Ftopsort(\Fordergraph(q), y)$.
We have that $(j, i)$ is an edge in $\Fordergraph(q)$, which implies that $\pi(j) < \pi(i)$ by Equation~\ref{eqn:topsort1}.
Because the elements of $y$ are sorted in descending order, and assumed to be distinct (Definition~\ref{def:safe-ordering}), we obtain that $y^s_{\pi(i)} < y^s_{\pi(j)}$, i.e., that $y'_i < y'_j$. 
\end{proof}

\begin{theorem}[\Fselfrepair is a self-repairing transformer]
\label{thm:sr-sound}
\Fselfrepair (Algorithm~\ref{alg:self_repair}) satisfies conditions \emph{(i)} and \emph{(ii)} of Definition~\ref{def:sr-transformer}.
\end{theorem}
\begin{proof}
By definition of Algorithm~\ref{alg:self_repair}, \linebreak
$\Fsolve(\Phi, x, y) = \bot$ if and only if $\arnet(x) = \Fselfrepair(\Phi)(f)(x)$ outputs $\bot$.
We derive from Property~\ref{thm:solvespec}\ref{thm:solvebot} that this is equivalent to
$\forall y'.~\lnot \Phi(x, y')$, which corresponds exactly to Property~\ref{def:sr-transformer}\ref{thm:forewarning}.
Conversely, if $\Phi$ is satisfiable for input $x$, i.e., $\exists y'.~\Phi(x, y')$,
then $\Fsolve(\Phi, x, y)$ outputs $q \neq \bot$.
By definition, we have $\arnet(x) = \Freorder(q, y)$, which satisfies $q$
by application of Property~\ref{thm:reorderspec}, which in turn implies
that $\Phi(x, \arnet(x))$ by application of
Property~\ref{thm:solvespec}\ref{thm:solverep}.
\end{proof}


\subsection{\ls`SR` is Transparent}
\label{sec:proof_transparency}

Now that we have demonstrated that our approach produces safe-by-construction networks,
we next prove that it also preserves predictions when possible, i.e.,
that \Fselfrepair satisfies \emph{transparency}, as formalized in Property~\ref{thm:transparency}.

Let $x : \mathbb{R}^n$ be an arbitrary vector.
As in the previous section, if $\Phi(x, f(x))$ is initially satisfied, transparency trivially
holds, as the repair layer does not modify the original output $f(x)$.
When $\Phi(x, f(x))$ does not hold, we will rely on several additional properties about \Fsolve, \Freorder, and \Fordergraph.
The first, Property~\ref{thm:tograph}, states that whenever the index of the network's prediction is a root of the graph encoding of $q$ used by \Fsolve and \Freorder, then there exists an output which satisfies $q$ that preserves that prediction.

\begin{Property}[\Fordergraph]
\label{thm:tograph}
Let $q$ be a satisfiable, disjunction-free ordering constraint,
and $y : \mathbb{R}^m$ a vector. Then,
\begin{align*}
\argmax_i\{y_i\} \in \rootg(\Fordergraph(q)) ~\Longleftrightarrow~\\
  \exists y'.~ q(y') ~\wedge~ \argmax_i\{y_i\} = \argmax_i\{y_i'\}
\end{align*}
\end{Property}

The intuition behind this property is that $i^* := \argmax_i\{y_i\}$ belongs to the roots
of $\Fordergraph(q)$ if and only if there is no $y_{i^*} < y_j$ constraint in $q$; hence
since $q$ is satisfiable, we can always permute indices in a solution $y'$ to have
$\argmax_i\{y'_i\} = i^*$.
%Building upon this intuition, we now prove
%that \Fsolve and \Freorder satisfy the properties outlined above, starting with \Fsolve, next.
Formally, Lemma~\ref{lem:topsort-invariant} in Section~\ref{sec:impl:stable_topological_sort} entails this property, as it shows that the permutation returned by \Ftopsort satisfies it.

Next, Property~\ref{thm:refinesolve} formalizes the requirement that whenever \Fsolve returns a constraint (rather than $\bot$), then that constraint will not eliminate any prediction-preserving solutions that would otherwise have been compatible with the full set of properties $\Phi.$

\begin{Property}[\Fsolve]
\label{thm:refinesolve}
Let $\Phi$ be a set of safety properties, $x : \mathbb{R}^n$ and $y : \mathbb{R}^m$ two vectors, and \linebreak $q = \Fsolve(\Phi, x, y)$. Then,
\begin{align*}
&q \neq \bot ~\wedge~ \left(\exists y'.~ \Phi(x, y') ~\wedge~ \argmax_i\{y_i\} = \argmax_i\{y_i'\}\right) \implies \\
&\exists y'.~q(y') ~\wedge~ \argmax_i\{y_i\} = \argmax_i\{y_i'\}
\end{align*}
\end{Property}
\begin{proof}
Let us assume that $q \neq \bot$, and that $\exists y'.~\Phi(x, y') \wedge \argmax_i\{y_i\} = \argmax_i\{y'_i\}$.
We will proceed by contradiction, assuming that there does not exist $y''$ such that
$q(y'')$ and $\argmax_i\{y_i\} = \argmax_i\{y''_i\}$, which
entails that $\argmax_i\{y_i\} \not\in \rootg(\Fordergraph(q))$
by application of Property~\ref{thm:tograph}.
In combination with the specification of \Fprioritize (Property~\ref{prop:prioritize}),
this implies that any $q' \in Q_p$ such that \linebreak
$\exists y'.~q'(y') \wedge \argmax_i\{y_i\} = \argmax_i\{y'_i\}$ occurs before $q$ in \linebreak
$\Fprioritize(Q_x, y)$, i.e., $\idx(q', Q_p) < \idx(q, Q_p)$.
From loop invariant~\ref{eqn:solve_loopinv}, we therefore conclude that there does
not exist such a $q' \in Q_p$, which contradicts the hypothesis $\Phi(x, y')$
by application of Equation~\ref{eqn:prspec}.
\end{proof}

Lastly, Property~\ref{thm:refinereorder} states that \Freorder (Algorithm~\ref{alg:repair:reorder}) will always find an output that preserves the original prediction, whenever the constraint returned by \Fsolve allows it.
This is the final piece needed to prove Theorem~\ref{thm:sr-transparency}, the desired result about the self-repairing transformer.

\begin{Property}[\Freorder]
\label{thm:refinereorder}
Let $q$ be a satisfiable term, and $y : \mathbb{R}^m$ a vector.
Then,
\begin{align*}
&(~\exists y'.~q(y') \wedge \argmax_i\{y_i\} = \argmax_i\{y_i'\}~)\\
&\implies \argmax_i\{\Freorder(q, y)_i\} = \argmax_i\{y_i\}
\end{align*}
\end{Property}
\begin{proof}
Assume that there exists $y'$ such that $q(y')$ and \linebreak
$\argmax_i\{y_i\} = \argmax_i\{y'_i\}$.
This entails that $\argmax_i(y_i) \in \rootg(\Fordergraph(q))$ (Property~\ref{thm:tograph}),
which in turn implies that $\pi(\argmax_i\{y_i\})$ is 0
(property~\ref{eqn:topsort2}).
By definition of a descending sort, we have that
$\argmax_i\{\Freorder(q, y)_i\} = j$, such that $\pi(j) = 0$,
hence concluding that $j = \argmax_i\{y_i\}$ by injectivity of $\pi$.
\end{proof}

\begin{theorem}[Transparency of \Fselfrepair]
\label{thm:sr-transparency}
\Fselfrepair, the self-repairing transformer described in Algorithm~\ref{alg:self_repair} satisfies Property~\ref{thm:transparency}.
\end{theorem}
\begin{proof}
That the \Fselfrepair transformer satisfies transparency is straightforward given Properties~\ref{thm:tograph}-\ref{thm:refinereorder}. 
Let us assume that there exists $y'$ such that
$\Phi(x, y')$ and $\argmax_i\{y'_i\} = F(x)$.
By application of Property~\ref{thm:solvespec}\ref{thm:solvebot},
this implies that \linebreak
$\Fsolve(\Phi, x, f(x))$ outputs $q \neq \bot$,
and therefore that there exists $y'$ such that $q(y')$ and $\argmax\{y'_i\} = F(x)$
by application of Property~\ref{thm:refinesolve}, since $F(x)$ is defined as $\argmax_i\{f_i(x)\}$.
Composing this fact with Property~\ref{thm:refinereorder}, we obtain that $F^\Phi(x) = F(x)$, since
$F^\Phi(x) = \argmax_i\{\arnet_i(x)\}$ by definition.
\end{proof}

%\af{Very hand-wavy}
%We first assume that $\argmax(y) \in Root(\Fordergraph(q))$.
%Let $g = \Fordergraph(q)$, and $i = \argmax(y)$.
%We consider the graph $g'$, where node $i$ and all corresponding edges were removed.
%Let $\pi$ be a topological sort of $g'$, i.e., $\pi$ maps indices to their rank (or position) in the total order.
%We define $y$ such that $\forall j. y'_j = \pi(j)$ 
%We then insert $m$ at index $i$.
%Since $i$ was a root of the original graph, and $\forall j. y'_i > y'_j$,
%and the resulting $y$ satisfies $q$.
%
%We now prove the other direction.
%Let $y'$ be such that $q(y') \wedge \argmax(y) = \argmax(y')$.
%We write $i = \argmax(y)$.
%Let us assume that $i \nsubseteq Root(\Fordergraph(q))$.
%By definition of $\Fordergraph$, there exists $j$ such that $y_i < y_j \in q$,
%which leads to a contradiction.


